Beyond Centrality: Understanding Urban Street Network Typologies Through Intersection Patterns

The structure of road networks plays a pivotal role in shaping transportation dynamics. It also provides insights into how drivers experience city streets and helps uncover each urban environment's unique characteristics and challenges. Consequently, characterizing cities based on their road network patterns can facilitate the identification of similarities and differences, informing collaborative traffic management strategies, particularly at a regional scale. While previous studies have investigated global network patterns for cities, they have often overlooked detailed characterizations within a single large urban region. Additionally, most existing research uses metrics like degree, centrality, orientation, etc., and misses the nuances of street networks at the intersection level, specifically the geometric angles formed by links at intersections, which could offer a more refined feature for characterization. To address these gaps, this study examines over 100 cities in the San Francisco Bay Area. We introduce a novel metric for classifying intersections, distinguishing between different types of 3-way and 4-way intersections based on the angles formed at the intersections. Through the application of clustering algorithms in machine learning, we have identified three distinct typologies - grid, orthogonal, and organic cities - within the San Francisco Bay Area. We demonstrate the effectiveness of the metric in capturing the differences between cities based on street and intersection patterns. The typologies generated in this study could offer valuable support for city planners and policymakers in crafting a range of practical strategies tailored to the complexities of each city's road network, covering aspects such as evacuation plans, traffic signage placements, and traffic signal control.

==> results_archive.tex <==
\section {Results}

In this section, we first present the results for baseline clustering, followed by enhanced clustering. We provide a comparison between the two to provide insights into the differences, In the baseline clustering, we identify six typologies, and the most important features are the link-node ratio, node degrees, and network density. 

\begin{figure}[ht]
  \includegraphics[width=.3\columnwidth]{figures/baseline_network_linknoderatio.png}\hfill
  \includegraphics[width=.3\columnwidth]
    {figures/baseline_network_degree1.png}\hfill
  \includegraphics[width=.3\columnwidth]
    {figures/baseline_network_degree3.png}\hfill
  \includegraphics[width=.3\columnwidth]
    {figures/baseline_network_degree4.png}\hfill
  \includegraphics[width=.3\columnwidth]
    {figures/baseline_median_betweeness.png}\hfill
  \includegraphics[width=.3\columnwidth]
  {figures/baseline_network_density.png}\hfill
  \caption{The figures show the summary of important features for the baseline network clusters.}
  \label{fig:stage2d}
\end{figure}


\begin{table}[ht]
\small
\centering
\caption{ Baseline Network Clusters}
\label{tab:metrics_streettype}
\begin{tabular}{|c|c|c|c|} 
\hline
\textbf{Clusters} &  \textbf{Features} & \textbf{Number of Cities}  & \textbf{Example Cities}  \\
\hline
\noalign{\smallskip}
0 & Low link-node ratio, High proportion & 6 & Tiburon, Los Altos Hills \\ 
 & of node degree 1, Low network density &     \\
2 & High link-node ratio, High proportion  & 6 & San Francisco, Berkeley\\ 
& of degree 4, High network density & \\

1 &  Medium link-node ratio, High proportion  & 12 & El Cerrito, Oakland \\ 
 &  of degree 3, Medium network density &  \\ 
3 & Medium link-node ratio, High proportion  & 27 & Santa Rosa, San Ramon\\
 &  of degree 3, Medium network density &  \\ 
4 & Medium link-node ratio,  Medium proportion   & 18 &  Milpitas, Palo Alto   \\
 & of degree 1, Medium network density, & \\
5 & Low link-node ratio, High proportion   & 24 & Fremont, Sonoma  \\
& of degree 1,  Low network density & \\
\noalign{\smallskip}
\hline
\end{tabular}
\end{table}


In the enhanced clustering, three typologies are identified, with the most important features being node degrees, node patterns, link-node ratio, and link bearings. By incorporating node patterns and link bearings, the level of differentiation is enhanced. 


\begin{figure}[ht]
\includegraphics[width=.25\columnwidth]
    {figures/nuanced_network_node_degree1.png}\hfill
  \includegraphics[width=.25\columnwidth]
    {figures/nuanced_network_node_degree3.png}\hfill
  \includegraphics[width=.25\columnwidth]
    {figures/nuanced_network_degree4.png}\hfill
      \includegraphics[width=.25\columnwidth]
{figures/nuanced_network_degree3_type1.png}\hfill
\includegraphics[width=.25\columnwidth]
{figures/nuanced_network_degree3_type2.png}\hfill
\includegraphics[width=.25\columnwidth]
{figures/nuanced_network_degree3_type3.png}\hfill
\includegraphics[width=.25\columnwidth]
{figures/nuanced_network_degree4_type1.png}\hfill
\includegraphics[width=.25\columnwidth]
{figures/nuanced_network_degree4_type2.png}\hfill
\includegraphics[width=.25\columnwidth]
{figures/nuanced_network_degree4_type3.png}\hfill
\includegraphics[width=.25\columnwidth]
    {figures/nuanced_network_linknoderatio.png}\hfill
  \includegraphics[width=.25\columnwidth]
    {figures/nuanced_network_b1.png}\hfill
  \includegraphics[width=.25\columnwidth]
{figures/nuanced_network_dominant_bearingbins.png}\hfill
    \caption{The figures show the summary of important features for the enhanced network clusters.}
  \label{fig:stage2d}
\end{figure}



\begin{table}[h]
\small
\centering
\caption{Enhanced Network Clusters}
\label{tab:metrics_streettype}
\begin{tabular}{|p{2.5cm}|p{4cm}|p{4cm}|p{4cm}} 
\hline
\textbf{Feature} &  \textbf{Cluster 2} & \textbf{Cluster 0}  & \textbf{Cluster 1}\\
\hline
\noalign{\smallskip}
\textbf{Node degree} & Highest prop of degree 4 nodes (4 way intersections)  & Highest prop of degree 3 nodes (3 way intersections) & Highest prop of degree 1 nodes (dead ends)  \\  
\textbf{Node pattern: Degree 3} & High proportion of Type 2 intersections & High proportion of Type 1 intersections (T intersections) & High proportion of non Type 1 intersections \\ 
\textbf{Node pattern: Degree 4} & High proportion of  Type 1   intersections & High proportion of  Type 1 and 3 intersections & No significant patterns \\
& & \\
\textbf{Link bearings} & High percentage of links are concentrated in a few specific bearing directions &  High percentage of links are concentrated in a few specific bearing directions & Links distributed in all bearing directions \\
& & \\
\textbf{Number of dominant bearing bins} & High number of dominant bearings bins (median 4) & High number of dominant bearings bins (median 4) & Few dominant bearing directions (median 0)\\
\textbf{Mean link length} & 132 & 140 & 150 \\ 
\textbf{Median Link node ratio}  & High & Medium & Low \\ 
\textbf{Number of Cities} & 17 & 35 & 41 \\
\textbf{Example Cities} & San Francisco, Berkeley & Cupertino, Los Altos & Los Altos Hills, Walnut Creek \\
\noalign{\smallskip}
\hline
\end{tabular}
\end{table}


\begin{figure}[ht]
  \includegraphics[width=.5\columnwidth]{figures/nuanced_network_examplecities_cluster0.png}\hfill
  \includegraphics[width=.5\columnwidth]
{figures/nuanced_network_examplecities_cluster1.png}\hfill
  \includegraphics[width=.5\columnwidth]
{figures/nuanced_network_examplecities_cluster2.png}\hfill
  \caption{The figures show the summary of important features for the baseline network clusters.}
  \label{fig:stage2d}
\end{figure}

\begin{figure}[h]
  \includegraphics[width=.5\columnwidth]
    {figures/baseline_network_clusters.png}
  \includegraphics[width=.5\columnwidth]
    {figures/nuanced_network_clusters.png}
  \caption{The figure shows the baseline (left) and enhanced (right) network-based city clusters }
  \label{fig:stage2c}
\end{figure}

For gridded cities, 
- Out-degree 3 type 1 highly correlated with degree 4. Gridded cities have one way streets. They also have high outdegree 2 since both one way streets. 





[2D - Cluster results PLOT]



